Foundation Model Engineering: Engineering Foundation Models Just as Engineering Software

By treating data and models as the source code, Foundation Models (FMs) become a new type of software. Mirroring the concept of software crisis, the increasing complexity of FMs making FM crisis a tangible concern in the coming decade, appealing for new theories and methodologies from the field of software engineering. In this paper, we outline our vision of introducing Foundation Model (FM) engineering, a strategic response to the anticipated FM crisis with principled engineering methodologies. FM engineering aims to mitigate potential issues in FM development and application through the introduction of declarative, automated, and unified programming interfaces for both data and model management, reducing the complexities involved in working with FMs by providing a more structured and intuitive process for developers. Through the establishment of FM engineering, we aim to provide a robust, automated, and extensible framework that addresses the imminent challenges, and discovering new research opportunities for the software engineering field.

==> threats.tex <==
\section{Threats to Validity}
The main external threats to the validity include the extent to which the subject apps and tools selected for our evaluation are representative of true practice.
This paper reports the experiences of developing and deploying automated UI testing tools at Honor, a highly popular mobile device vendor. 

The threats to internal validity are instrumentation effects that can bias our results, including faults in our implementation of \toolname{}, parameter selection of \toolname{}, and randomness.
To reduce the randomness of experiments, we run all test tools on each app three times following previous work to mitigate the issue.


